Counting and Computing Join-Endomorphisms in Lattices (Revisited)

Structures involving a lattice and join-endomorphisms on it are ubiquitous in computer science. We study the cardinality of the set $\mathcal{E}(L)$ of all join-endomorphisms of a given finite lattice $L$. In particular, we show for $\mathbf{M}_n$, the discrete order of $n$ elements extended with top and bottom, $| \mathcal{E}(\mathbf{M}_n) | =n!\mathcal{L}_n(-1)+(n+1)^2$ where $\mathcal{L}_n(x)$ is the Laguerre polynomial of degree $n$. We also study the following problem: Given a lattice $L$ of size $n$ and a set $S\subseteq \mathcal{E}(L)$ of size $m$, find the greatest lower bound ${\large\sqcap}_{\mathcal{E}(L)} S$. The join-endomorphism ${\large\sqcap}_{\mathcal{E}(L)} S$ has meaningful interpretations in epistemic logic, distributed systems, and Aumann structures. We show that this problem can be solved with worst-case time complexity in $O(mn)$ for distributive lattices and $O(mn + n^3)$ for arbitrary lattices. In the particular case of modular lattices, we present an adaptation of the latter algorithm that reduces its average time complexity. We provide theoretical and experimental results to support this enhancement. The complexity is expressed in terms of the basic binary lattice operations performed by the algorithm.

==> Body/subsec-proof-lemma3-sergio.tex <==
% !TeX root = ../main.tex


\subsection{Proof of Theorem~\ref{size4m-n:lemma}.}
\label{app:proof-count-Mn}

We shall show that $|\sfunspace{\M_n}|$ can be expressed in terms of Laguerre polynomials:
\( |\sfunspace{\M_n}| = (n+1)^2  +  n! \laguerre{n}{-1}\).

Let $\fcal = \bigcup_{i=1}^4\fcal_i$ where the mutually exclusive $\fcal_i$'s
are defined in Table~\ref{sfunc-mn-red:table}, and $I=\{1,\ldots,n\}$. The proof is divided in two parts: (I) $\sfunspace{\M_n} = \fcal$
and (II) $|\fcal| = (n+1)^2  +  n! \laguerre{n}{-1}.$

\subsubsection{Part (I)} For $\fcal \subseteq \sfunspace{\M_n}$, it is easy to verify that each $f \in \fcal$ is a join-endomorphism.

For $\sfunspace{\M_n} \subseteq \fcal$ we show that for any function $f$ from $\M_n$ to $\M_n$  if $f \not\in \fcal$, then $f \not\in \sfunspace{\M_n}$. Immediately, if $f(\bot)\neq \bot$ then $f \not\in  \sfunspace{\M_n}$. 

Suppose $f(\bot) = \bot$.
Let $J, K, H$ be disjoint possibly empty sets such that $I = J \cup K \cup H$ and
let $j= |J|$, $k = |K|$ and $h = |H|$. The sets $J, K, H$ represent the elements of $I$ mapped by $f$ to $\top$,  
to elements of $I$, and to $\bot$, resp. More precisely,
$\mathrm{Img}(\fres{f}{J}) = \{\top\}$,
$\mathrm{Img}(\fres{f}{K}) \subseteq I$ and
$\mathrm{Img}(\fres{f}{H}) = \{\bot\}$.
Furthermore, for every $f$ either (1) $f(\top) = \bot$, (2) $f(\top) \in I$ or (3) $f(\top) = \top$. For each case we show that $f \not\in  \sfunspace{\M_n}$. 

\begin{enumerate}
\item $f(\top) = \bot$. Since $f \not\in \fcal_1$ there is an $e \in I$ such that $f(e) \neq \bot$. We have $e \cleq \top$ but $f(e) \not\cleq f(\top)$. Then $f$ is not monotonic.
From Prop. \ref{prop:monotonicity} we conclude  $f \not\in \sfunspace{\M_n}$.

\item $f(\top) \in I$. Let $K_1,K_2$ be disjoint possibly empty sets such that $K_1 \cup K_2 = K$,
$\mathrm{Img}(\fres{f}{K_1}) = \{f(\top)\}$ and
$\mathrm{Img}(\fres{f}{K_2}) \neq \{f(\top)\}$.
Notice that if $j > 0$ or $|K_2| > 0$, $f$ is non-monotonic and then
$f \not\in \sfunspace{\M_n}$.

We then must have $j = 0$ and $K_2 = \emptyset$. Since $\mathrm{Img}(\fres{f}{K})
= \{f(\top)\}$ and $f \not\in \fcal_2$ then $h > 1$. Therefore there must be
$e_1, e_2 \in H$ such that $f(e_1) = f(e_2) = \bot$. This implies
$f(e_1 \join e_2) = f(\top) \neq \bot = f(e_1) \join f(e_2)$, therefore $f \not\in \sfunspace{\M_n}$.

\item $f(\top) = \top$. 

\begin{enumerate}[label*=\arabic*.]
\item Suppose $k = 0$. Notice that $f \not\in \fcal_3$ and $f \not\in \fcal_4$
hence $h \neq 1$ and $h \neq 0$. Thus $h >1$ implies that
there are at least two $e_1, e_2 \in H$ such that $f(e_1) = f(e_2) = \bot.$
But then  $f(e_1 \join e_2) = f(\top) = \top \neq \bot = f(e_1) \join f(e_2)$,
hence $f \not\in \sfunspace{\M_n}$.


\item Suppose $k > 0$.
Assume $h=0.$ Let $K_1, K_2$ be disjoint possibly empty sets
such that $K_1 \cup K_2 = K$, $\mathrm{Img}(\fres{f}{K_1}) \subseteq J$ 
and $\mathrm{Img}(\fres{f}{K_2}) \subseteq I \setminus J$. 
Notice that $f$ is a  $\bot$ and $\top$ preserving function and satisfies conditions (a) and (c)
of $\fcal_4$ but   $f \not\in \fcal_4$, then $f$ must violate condition (b). Thus $\fres{f}{K_1}$ or
$\fres{f}{K_2}$ is not injective. Let us assume that  $\fres{f}{K_1}$ is not injective (the case when 
$\fres{f}{K_2}$
is not injective is analogous). 
Then there are $a,b \in K_1$ and $c \in J$, such that
$a \neq b$ but $f(a) = f(b) = c$. By definition
$\top \not\in J$, then $f(a) \join f(b) = c \neq \top = f(a \join b)$. Consequently, $f \not\in \sfunspace{\M_n}$.


Assume $h>0$. There must be $e_1, e_2, e_3 \in I$  such that $f(e_1) = \bot$
and $f(e_2) = e_3$. Notice $e_1 \join e_2 = \top$, we then have 
$f(e_1) \join f(e_2) = e_3 \neq \top = f(e_1 \join e_2)$. Therefore, 
$f \not\in \sfunspace{\M_n}$.
\end{enumerate} 

% Since $f \not\in \fcal_2$, from condition (b) we know that for all
% $e_1,e_2 \in I$, $f(e_1) \neq \bot$ and $f(e_2) \neq e_1$.
% Taking $e_1 = e$ and $e_2 = e'$, we have $f(e) \neq \bot$ and
% $f(e') \neq e$. Notice that $f(e \join \top) = e'$ and
% $f(e) \join f(\top) = f(e) \join e'$, where $f(e) \neq e'$ and
% $f(e) \neq \bot$. Then $f(e) \join e' = \top$ and $f(e \join \top)
% \neq f(e) \join f(\top)$. Therefore $f \not\in \sfunspace{\M_n}$.


\end{enumerate}

\subsubsection{Part (II)} We prove that $|\fcal| = \sum_{i=1}^4|\fcal_i| = (n+1)^2  +  n! \laguerre{n}{-1}$.
Recall that $n = |I|$.

\begin{enumerate}
\item $|\fcal_1| = 1$.
There is only one function mapping every element in $\M_n$ to $\bot$.

\item $|\fcal_2| = n^2 + n$.
Since $\top$ is mapped to an element of $I$, there are $n$ 
possibilities to choose such element. If there is an element of $I$ mapped to
$\bot$, for each one of the previous $n$ options there are also $n$
possibilities to choose an element of $I$ to be mapped to $\bot$.
Then, in this case there are $n^2$ functions. If no element of $I$
is mapped to $\bot$, then there are $n$ additional functions.

\item $|\fcal_3| = n$. One of the elements of $I$ is mapped to $\bot$.
All the other elements of $I$ are mapped to $\top$. Then, there are $n$ 
functions that can be defined in $\fcal_3$.

\item $|\fcal_4| = \Rook{n}{1}$.
Let $f \in \fcal_4$ and let $J, K_1, K_2$ be disjoint possibly empty sets 
such that $I = J \cup K_1 \cup K_2$,
$\mathrm{Img}(\fres{f}{J}) = \{\top\}$,
$\mathrm{Img}(\fres{f}{K_1}) \subseteq J$ and
$\mathrm{Img}(\fres{f}{K_2}) \subseteq I \setminus J$, where
$\fres{f}{K_1}$ and $\fres{f}{K_2}$ are injective functions.
We shall call $j = |J|$ and $k_1 = |K_1|$.
% Note that $|K_2| = n-j-k_1$.

%Now, there are $\binom{n}{j}$ possibilities to choose $J$ among the 
%elements of $I$. For each choice of $J$, the elements of $K_1$ are to be 
%mapped to elements of $J$ by the injective function $\fres{f}{K_1}$.
%This is possible only if $k_1\leq j$, then we take $k_1 \leq \min(j,n-j)$.
%The number of choices of $K_1$ is $\binom{n-j}{k_1}$ and the number of choices
%among $J$ that can be targets of the elements of $K_1$ is $\binom{j}{k_1}$.
%Each of this can be targeted by any permutation of $K_1$, then we have 
%$\binom{j}{k_1}k_1! = \frac{j!}{(j-k_1)!}$ possibilities to choose $K_1$
%and map its elements by $\fres{f}{K_1}$ to elements of $J$. Similarly,
%the number of possibilities to choose $K_2$ and map its elements
%by $\fres{f}{K_2}$ to elements of $I \setminus J$ is
%$\binom{n-j}{n-j-k_1}(n-j-k_1)! = \frac{(n-j)!}{k_1!}$.
%Therefore, $|\fcal_4| = \sum_{j=0}^{n}\binom{n}{j} \sum_{k_1=0}^{\min(j,n-j)}
%\binom{n-j}{k_1}\frac{j!}{(j-k_1)!}\frac{(n-j)!}{k_1!}$.


For each of the $\binom{n}{j}$ possibilities  for $J$, the elements of $K_1$ are to be 
mapped to them by the injective function $\fres{f}{K_1}$.
This is possible only if $k_1\leq j$, so we take $k_1 \leq \min(j,n-j)$.
The number of choices of $K_1$ is $\binom{n-j}{k_1}$ and the number of choices
among $J$ that can be targets of those is $\binom{j}{k_1}$.
Each of these can be mapped from any permutation of $K_1$, so we have 
$\binom{j}{k_1}k_1! = \frac{j!}{(j-k_1)!}$ possibilities to choose $K_1$
and map its elements by $\fres{f}{K_1}$ to elements of $J$. Similarly,
the number of possibilities to choose $K_2$ and map its elements
by $\fres{f}{K_2}$ to elements of $I \setminus J$ is
$\binom{n-j}{n-j-k_1}(n-j-k_1)! = \frac{(n-j)!}{k_1!}$.
Therefore, $|\fcal_4| = \sum_{j=0}^{n}\binom{n}{j} \sum_{k_1=0}^{\min(j,n-j)}
\binom{n-j}{k_1}\frac{j!}{(j-k_1)!}\frac{(n-j)!}{k_1!}$.
We can simplify the inner sum:
\( \sum_{k_1=0}^{\min(j,n-j)} \binom{n-j}{k_1}\frac{j!}{(j-k_1)!}\frac{(n-j)!}{k_1!}
= \frac{n!}{j!}\).
We then obtain  $|\fcal_4| = \sum_{j=0}^{n}\binom{n}{j}
\frac{n!}{j!}$. This sum equals $n!\laguerre{n}{-1}$ which in turn 
is equal  to $\Rook{n}{1}.$

\end{enumerate}

It follows that $|\fcal| = \sum_{i=1}^4|\fcal_i| = (n + 1)^2 + n! \laguerre{n}{-1} $ as wanted. 
\qed

% \subsubsection{Proof of Theorem~\ref{rook:th}.}
% We wish to prove that $| A | = \Rook{n}{1}$ where $ A=  \{ \ f \in \sfunspace{\M_n} \mid f \mbox{ is non-reducing in }  \M_n \ \} $. Let $\fcal = \bigcup_{i=1}^4\fcal_i$ where the mutually exclusive $\fcal_i$'s
% are defined in Table~\ref{sfunc-mn-red:table}. In the proof of Theorem~\ref{size4m-n:lemma} we show that $\sfunspace{\M_n} = \fcal$ and that  $\Rook{n}{1} = |\fcal_4|$.  Notice that every function in $\fcal_4$ is non-reducing and every function in $\fcal \setminus \fcal_4$ is not non-reducing. Hence $A = \fcal_4$, thus $ | A | = \Rook{n}{1}.$




==> Body/subsec-proof-lemma4-sergio.tex <==
% !TeX root = ../main.tex


\subsection{Proof of Lemma~\ref{lemma:delta-ast}}

Let  $\Lat$ be a finite distributive lattice and
$S = \{ f_i \}_{i \in I} \subseteq \sfunspace{L}$.
Then
\( \Dfun{S}  = \dplusfun{S} \mbox {\ where \ } \dplusfunapp{S}{c}
\defsymbol \bigmeetp{\Lat}\{ \bigjoin_{i \in I}\sfunapp{i}{a_i}
\ | \ (a_i)_{i \in I} \in \tuplespace{\Con}{I} \mbox { and }\
\bigjoin_{i \in I}{a_i} \cgeq c \}.\)

\begin{proof}
	Recall that $\Dfun{S} = \textit{max}\{ h \in \jhspace{\Lat} \ |\
	h \hleq g \mbox{ for all } g \in S\}$ and let us define
 $\Gamma = \{ \bigjoin_{i \in I}\sfunapp{i}{a_i} \ | \ 
 (a_i)_{i \in I} \in \tuplespace{\Con}{I} \mbox { and }\
 \bigjoin_{i \in I}{a_i} \cgeq c \}$.
	We prove (1) $\Dfun{S} \hleq \dplusfun{S}$ and (2) $\dplusfun{S} \hleq \Dfun{S}$.

	\begin{enumerate}
		\item $\Dfun{S} \hleq \dplusfun{S}$.

		Let $c \in \Con$ and $(a_i)_{i \in I} \in \tuplespace{\Con}{I}$
		be an arbitrary tuple such that $\bigjoin_{i \in I}{a_i} \cgeq c$.
		Notice that $\bigjoin_{i\in I}\Dfunapp{S}{a_i}
    \cleq \bigjoin_{i\in I}\sfunapp{i}{a_i}$. Since $\Dfun{S}$ is a
    join-endomorphism of $\Lat$ and monotonic, we know that
    $\bigjoin_{i\in I}\Dfunapp{S}{a_i}
    = \Dfunapp{S}{\bigjoin_{i\in I} a_i} \cgeq \Dfunapp{S}{c}$.
    Thus $\Dfunapp{S}{c} \cleq \bigjoin_{i\in I}\sfunapp{i}{a_i}$, i.e.
    $\Dfunapp{S}{c}$ is a lower bound of $\Gamma$.
		Then for every $c \in \Con$, $\Dfunapp{S}{c} \cleq
		\dplusfunapp{S}{c}$. Therefore $\Dfun{S} \hleq \dplusfun{S}$.
		
		\item $\dplusfun{S} \hleq \Dfun{S}$.

		We prove (a) $\dplusfun{S} \in \jhspace{\Lat}$ and
		(b) $\dplusfun{S} \hleq \sfun{i}$ for every $\sfun{i} \in S$.

		\begin{enumerate}
			\item Prove that $\dplusfun{S} \hleq \sfun{i}$, for every $\sfun{i} \in S$.

			Let $c \in \Con$.
      From definition of $\dplusfun{S}$, for every $i \in I$, the element
      $\sfunapp{i}{c} = \sfunapp{i}{c} \join \bigjoin_{j \in I \setminus \{i\}}
      \sfunapp{j}{\bot} \in \Gamma$.
			Then for every $c \in \Con$, $\dplusfunapp{S}{c} \cleq \sfunapp{i}{c}$.
			Therefore for every $\sfun{i} \in S$, $\dplusfun{S} \hleq \sfun{i}$.
			
			\item $\dplusfun{S} \in \jhspace{\Lat}$.

			We show that for any $H \subseteq L$, $\dplusfunapp{S}{\bigjoin H} =
			\bigjoin\{ \dplusfunapp{S}{e}\ |\ \text{ for every } e \in H \}$.
      Since $H$ is finite, it suffices to show that our claim holds for
      $H = \emptyset$ and $H = \{c, d\}$.

			Assume $H = \emptyset$. One can verify that $\dplusfunapp{S}{\bot} = \bot$.

			Assume $H = \{c, d\}$. Firstly, we prove that $\dplusfun{S}$ is monotonic. 
			Suppose $c \cgeq d$. For any $(a_i)_{i \in I} \in \tuplespace{\Con}{I}$ 
			such that $\bigjoin_{i \in I}{a_i} \cgeq c$, we have
			$\bigjoin_{i \in I}{a_i} \cgeq d$.
			Therefore, $\{ \bigjoin_{i \in I}\sfunapp{i}{a_i}\
			|\ \bigjoin_{i \in I}{a_i} \cgeq c \} \subseteq \{ \bigjoin_{i \in I}
			\sfunapp{i}{a_i}\ |\ \bigjoin_{i \in I}{a_i} \cgeq d \}$ which implies
			$\dplusfunapp{S}{c} \cgeq \dplusfunapp{S}{d}$.

			By monotonicity of $\dplusfun{S}$, we know $\dplusfunapp{S}{c \join d}
			\cgeq \dplusfunapp{S}{c} \join \dplusfunapp{S}{d}$. The other direction
			follows from the derivation below:

			\begin{align*}
			&
			\dplusfunapp{S}{c} \join \dplusfunapp{S}{d}\\
			=\
			&
			\expl{\text{Definition of } \dplusfunapp{S}{d}}\\
			&
			\dplusfunapp{S}{c} \join \bigmeetp{\Lat}\{ \bigjoin_{i \in I}\sfunapp{i}{b_i} \ |\ (b_i)_{i \in I} \in \tuplespace{\Con}{I} \mbox{ and } \bigjoin_{i \in I}{b_i} \cgeq d \}\\
			=\
			&
			\expl{\join \text{ distributes over } \meet}\\
			&
			\bigmeetp{\Lat}\{ \dplusfunapp{S}{c} \join \bigjoin_{i \in I}\sfunapp{i}{b_i} \ |\ (b_i)_{i \in I} \in \tuplespace{\Con}{I} \mbox{ and } \bigjoin_{i \in I}{b_i} \cgeq d \}\\
			=\
			&
			\expl{\text{Definition of } \dplusfunapp{S}{c}}\\
			&
			\bigmeetp{\Lat}\{ \bigmeetp{\Lat}\{ \bigjoin_{i \in I}\sfunapp{i}{a_i} \ |\ (a_i)_{i \in I} \in \tuplespace{\Con}{I} \mbox{ and } \bigjoin_{i \in I}{a_i} \cgeq c \} \join \bigjoin_{i \in I}\sfunapp{i}{b_i} \ |\ (b_i)_{i \in I} \in \tuplespace{\Con}{I} \mbox{ and } \bigjoin_{i \in I}{b_i} \cgeq d \}\\
			=\
			&
			\expl{\join \text{ distributes over } \meet}\\
			&
			\bigmeetp{\Lat}\{ \bigmeetp{\Lat}\{ \bigjoin_{i \in I}\sfunapp{i}{a_i} \join \bigjoin_{i \in I} \sfunapp{i}{b_i} \ |\ (a_i)_{i \in I} \in \tuplespace{\Con}{I} \mbox{ and } \bigjoin_{i \in I}{a_i} \cgeq c \} \ |\ (b_i)_{i \in I} \in \tuplespace{\Con}{I} \mbox{ and } \bigjoin_{i \in I}{b_i} \cgeq d \}\\
			=\
			&
			\expl{ \text{Associativity of } \meet }\\
			&
			\bigmeetp{\Lat}\{ \bigjoin_{i \in I} (\sfunapp{i}{a_i} \join \sfunapp{i}{b_i}) \ |\ (a_i)_{i \in I}, (b_i)_{i \in I} \in \tuplespace{\Con}{I} \mbox{ and } \bigjoin_{i \in I}{a_i} \cgeq c \text{ and } \bigjoin_{i \in I}{b_i} \cgeq d \}\\
			\cgeq
			&
			\expl{ x \cgeq y \text{ and } w \cgeq z \text{ implies } x \join w \cgeq y \join z;\ c_i = a_i \join b_i;\ \sfunapp{i}{c_i} = \sfunapp{i}{a_i \join b_i}}\\
			&
			\bigmeetp{\Lat}\{\bigjoin_{i \in I} \sfunapp{i}{c_i} \ |\ (c_i)_{i \in I} \in \tuplespace{\Con}{I} \mbox{ and } \bigjoin_{i \in I}{c_i} \cgeq c \join d \}\\
			=\
			&
			\expl{\text{Definition of } \dplusfunapp{S}{ c \join d}}\\
			&
			\dplusfunapp{S}{c \join d}
			\end{align*}

			Thus we conclude $\dplusfun{S} \in \jhspace{\Lat}$.
		\end{enumerate}
		From items (a) and (b), $\dplusfun{S} \hleq \Dfun{S}$ holds.
	\end{enumerate}
 We conclude $\Dfun{S} = \dplusfun{S}$.
\end{proof}

\subsection{Proof of Corollary~\ref{rook:th}.}
We wish to prove that $| A | = \Rook{n}{1}$ where $ A=  \{ \ f \in \sfunspace{\M_n} \mid f \mbox{ is non-reducing in }  \M_n \ \} $. Let $\fcal = \bigcup_{i=1}^4\fcal_i$ where the mutually exclusive $\fcal_i$'s
are defined in Table~\ref{sfunc-mn-red:table}. In the proof of Theorem~\ref{size4m-n:lemma} we show that $\sfunspace{\M_n} = \fcal$ and that  $\Rook{n}{1} = |\fcal_4|$.  Notice that every function in $\fcal_4$ is non-reducing and every function in $\fcal \setminus \fcal_4$ is not non-reducing. Hence $A = \fcal_4$, thus $ | A | = \Rook{n}{1}$.



==> Body/subsec-proof-thm-camilo.tex <==
% !TeX root = ../main.tex

\subsection{Proof of Theorem~\ref{theorem:approx-correct}}
Let  $L$ be a finite  lattice, $u,v\in \Lat$, $\dapprox: \Con \rightarrow \Con$ and  $S \subseteq \sfunspace{L}$. Assume  $\dapprox \cgeq \Dfun{S}$ holds, and consider the following updates:
\begin{enumerate}
\item  when $\dapprox(u)
\join\dapprox(v)\cl\dapprox(u\join v)$, assign
$\dapprox(u\join v) \leftarrow \dapprox(u)\join\dapprox(v)$
\item when
$\dapprox(u)\join\dapprox(v)\not\cleq\dapprox(u\join v)$, assign
$\dapprox(u)\gets \dapprox(u)\meet\dapprox(u\join v)$ and also 
$\dapprox(v)\gets \dapprox(v)\meet\dapprox(u\join v)$
\end{enumerate}
Let $\dapprox'$ be the function resulting after the update. Then, (1) $\dapprox' \cl \dapprox$ and (2) $\dapprox' \cgeq \Dfun{S}$

\begin{proof}
For update (1):\\
 given the condition, the assignment obviously decreases $\dapprox(u\join v)$, so $\dapprox' \cl \dapprox$. For the invariant, since $\dapprox\cgeq \Dfun{S}$, then,
$\dapprox(u)\cgeq   \Dfunapp{S}{u}$ and $\dapprox(v)\cgeq   \Dfunapp{S}{v}$, and therefore,
 $ \dapprox'(u\join v)=\dapprox(u)\join \dapprox(v) \cgeq \Dfunapp{S}{u}\join \Dfunapp{S}{v} = \Dfunapp{S}{u\join v}$.
  
For update (2),\\ the assignments either decrease $\dapprox(u)$ or $\dapprox(v)$ (or both). To see why, assume the opposite, 
$ \dapprox(u) = \dapprox(u)\meet\dapprox(u\join v) \imp \dapprox(u) \cleq \dapprox(u\join v) $,  and also $\dapprox(v) = \dapprox(v)\meet\dapprox(u\join v) \imp \dapprox(v) \cleq \dapprox(u\join v) $. Therefore, $  \dapprox(u)\join\dapprox(v) \cleq \dapprox(u\join v)$, 
contradicting the condition for update 2. Assignments in update 2 also preserve the invariant $\dapprox\cgeq \Dfun{S}$.

assume $ \dapprox(u)\meet\dapprox(u\join v)\cl \dapprox(u)$ (otherwise the invariant holds trivially). By the invariant hypothesis for $\dapprox$ before the assignment, we have that $ \dapprox(u) \cgeq \Dfunapp{S}{u}$ and $ \dapprox(u\join v) \cgeq \Dfunapp{S}{u\join v}$. Therefore, 
\[
\begin{array}{ll}
%   \dapprox(u) \cgeq \Dfunapp{I}{u}&\\
%   \dapprox(u\join v) \cgeq \Dfunapp{I}{u\join v}&\\
\dapprox(u)\meet\dapprox(u\join v) &\cgeq \Dfunapp{S}{u}\meet\Dfunapp{S}{u\join v}\\
&= \Dfunapp{S}{u}\meet(\Dfunapp{S}{u}\join \Dfunapp{S}{v})\\
&=
% \Dfunapp{S}{u}\meet(\Dfunapp{S}{u}\join \Dfunapp{S}{v})\\
\Dfunapp{S}{u}\join(\Dfunapp{S}{u}\meet \Dfunapp{S}{v})\\
&=\Dfunapp{S}{u}
\end{array}
\]
The proof for $\dapprox'(v)$ is analogous.
%By the invariant hypothesis for $\dapprox$ before the assignment, we have that $ \dapprox(u) \cgeq \Dfunapp{S}{u}$ and $ \dapprox(u\join v) \cgeq \Dfunapp{S}{u\join v}$. Therefore,  $\dapprox'(u)=\dapprox(u)\meet\dapprox(u\join v)\cgeq  \Dfunapp{S}{u}\meet\Dfunapp{S}{u\join v}$. Now, since $\Dfun{S}$ distributes over joins, we have that $\Dfunapp{S}{u}\meet\Dfunapp{S}{u\join v} = \Dfunapp{S}{u}\meet(\Dfunapp{S}{u}\join \Dfunapp{S}{v})$ and also $\Dfunapp{S}{u}\meet(\Dfunapp{S}{u}\join \Dfunapp{S}{v})= \Dfunapp{S}{u}\join(\Dfunapp{S}{u}\meet \Dfunapp{S}{v})$, which, by the properties of $\meet$ and $\join$, is equal to $\Dfunapp{S }{u}$.

\end{proof}



==> Body/subsec-proof-thm2-sergio.tex <==
% !TeX root = ../main.tex

\subsection{Proof of Corollary~\ref{cor:rec1}}

Let $({\Con},\cleq)$ be a finite distributive lattice and
$S = \{ f_i \}_{i \in I} \subseteq \sfunspace{L}$.
Let $S_1,S_2 \subseteq \sfunspace{L}$ be such that
$S = S_1 \cup S_2$. Then 
\[
\Dfunapp{S}{c} = \bigmeetp{\Lat}\{ \Dfunapp{S_1}{a} \join \Dfunapp{S_2}{b}
\ |\ a \join b \cgeq c \}.
\]

\begin{proof}
The proof follows using the fact that $\Dfun{S} \in \sfunspace{L}$
and Lemma~\ref{lemma:delta-ast}.

Let $a,b,c \in \Con$ such that $a \join b \cleq c$.
Let $S_1 = \{ f_j \}_{j \in J}$ and $S_2 = \{ f_k \}_{k \in K}$ such
that $I = J \cup K$.
From Lemma~\ref{lemma:delta-ast}
%
\[
\Dfunapp{S_1}{a} = \bigmeetp{\Lat}\{ \bigjoin_{j \in J}
\sfunapp{j}{a_j} \ | \ (a_j)_{j \in J} \in \tuplespace{\Con}{J}
\mbox { and } \ \bigjoin_{j \in J}{a_j} \cgeq a \}\\
\]
%
and
%
\[
\Dfunapp{S_2}{b} = \bigmeetp{\Lat}\{ \bigjoin_{k \in K}
\sfunapp{k}{b_k} \ | \ (b_k)_{k \in K} \in \tuplespace{\Con}{K} \mbox { and }
\ \bigjoin_{k \in K}{b_k} \cgeq b \}.
\]
%
By distributivity of $\join$ over $\meet$, $\Dfunapp{S_1}{a} \join \Dfunapp{S_2}{b}$
can be written as:
%
\[
\bigmeetp{\Lat}\{ \bigjoin_{i \in I} \sfunapp{i}{c_i} \ | \ (c_i)_{i \in I} \in \tuplespace{\Con}{I}
\mbox { and }\ \bigjoin_{i \in I}{c_i} \cgeq a \join b \}
\]
%
where $c_i$ is either $a_i$, $b_i$ or $a_i \join b_i$.
\begin{align*}
&
\bigmeetp{\Lat} \{\Dfunapp{S_1}{a} \join \Dfunapp{S_2}{b}\ |\ a \join b \cgeq c\}\\
=&
\expl{\text{Construction of } \Dfunapp{S_1}{a} \join \Dfunapp{S_2}{b}} \\
&
\bigmeetp{\Lat} \{ \bigmeetp{\Lat}\{ \bigjoin_{i \in I} \sfunapp{i}{c_i} \ | \ (c_i)_{i \in I} \in
\tuplespace{\Con}{I} \mbox { and }\ \bigjoin_{i \in I}{c_i} \cgeq a \join b \}\
|\ a \join b \cgeq c\}\\
=&
\expl{\text{Associativity of } \meet} \\
&
\bigmeetp{\Lat}\{ \bigjoin_{i \in I} \sfunapp{i}{c_i} \ | \ (c_i)_{i \in I} \in
\tuplespace{\Con}{I} \mbox{ and }\ \bigjoin_{i \in I}{c_i} \cgeq a \join b \mbox{ and }
a \join b \cgeq c\}\\
=&
\expl{(\cgeq) \text{Transitivity of } \cgeq;\ (\cleq) \text{Associativity of } \meet.}\\
&
\bigmeetp{\Lat}\{ \bigjoin_{i \in I} \sfunapp{i}{c_i} \ | \ (c_i)_{i \in I} \in
\tuplespace{\Con}{I} \mbox{ and }\ \bigjoin_{i \in I}{c_i} \cgeq c\}\\
=&
\expl{\text{Lemma~\ref{lemma:delta-ast}}}\\ 
&
\Dfunapp{S}{c}
\end{align*}
\end{proof}

\subsection{Proof of Theorem~\ref{thm:comp-algo}}

Suppose  $({\Con},\cleq)$ is a finite distributive lattice.
Let $S_1,S_2 \subseteq \sfunspace{L}$ be such that
$S = S_1 \cup S_2 \subseteq \sfunspace{L}$. Then 
\[
\Dfunapp{S}{c}  =  \bigmeetp{\Lat}\{ \Dfunapp{S_1}{a} \join 
\Dfunapp{S_2}{c \latminus a} \mid a \in \Con \ \mbox{ and } \ a \cleq c \} .
\]

\begin{proof}
Firstly, we prove that
\begin{equation}
\label{eq:aux}
\Dfunapp{S}{c} =  \bigmeetp{\Lat}\{ \Dfunapp{S_1}{a} \join \Dfunapp{S_2}{c \latminus a }\}.
\end{equation}
From its definition $c \latminus a$ represents the least element $e$ such that 
$a \join e \cgeq c$, i.e.$c \latminus a = \bigmeet\{ e |  a \join e \cgeq c  \} $. Take any $b$ such that $a \join b \cgeq c$.
Then $b \cgeq c \latminus a$ and since $\Dfun{S_1}$ and $\Dfun{S_2}$
are monotonic
\[
\Dfunapp{S_1}{a} \join  \Dfunapp{S_2}{b} \cgeq \Dfunapp{S_1}{a}
\join \Dfunapp{S_2}{c \latminus a}.
\]
From this it follows that
\begin{align*}
& \bigmeetp{\Lat} ( C \cup \{ \Dfunapp{S_1}{a} \join  \Dfunapp{S_2}{c \latminus a }\ ,
\Dfunapp{S_1}{a} \join \Dfunapp{S_2}{b} \})\\
= &\bigmeetp{\Lat} ( C \cup \{ \Dfunapp{S_1}{a} \join \Dfunapp{S_2}{c \latminus a } \})
\end{align*}
for any $C \subseteq \Con$.
This shows that $\Dfunapp{S_1}{a} \join  \Dfunapp{S_2}{b}$ is redundant since
$\Dfunapp{S_1}{a} \join  \Dfunapp{S_2}{c \latminus a }$ is included in the set on the
right-hand side of Equation~\ref{eq:aux}.

The theorem can be seen as a simplification of Equation~\ref{eq:aux}.
Take any $a' \not\cleq c$. It suffices to find $a \cleq c$ such that
\[
\Dfunapp{S_1}{a'} \join \Dfunapp{S_2}{c \latminus a' } \cgeq
\Dfunapp{S_1}{a} \join \Dfunapp{S_2}{c \latminus a }
\]
since then for any $C \subseteq \Con$
\begin{align*}
&\bigmeetp{\Lat} ( C \cup \{ \Dfunapp{S_1}{a} \join \Dfunapp{S_2}{c \latminus a },\ \Dfunapp{S_1}{a'}
\join \Dfunapp{S_2}{c \latminus a' } \})\\
&= \bigmeetp{\Lat} ( C \cup \{ \Dfunapp{S_1}{a} \join \Dfunapp{S_2}{c \latminus a } \}).
\end{align*}
Since $a' \not\cleq c$ either (a) $a' \cg c$ or 
(b) $a'$ and $c$ are incomparable w.r.t. $\cleq$, written $a' \parallel c$.
Suppose (a) holds. Then take $a = c$ thus $c \latminus a = true$.
By monotonicity we have $ \Dfunapp{S_1}{a'} \join \Dfunapp{S_2}{c \latminus a' } \cgeq 
\Dfunapp{S_1}{a} \join  \Dfunapp{S_2}{c \latminus a }$ as wanted.
Suppose that (b) $a' \parallel c$ holds. Notice that $c \latminus a' \cleq c$.
Suppose that $c \latminus a' = c$. Then we can take $a = \true$, and thus
$c \latminus a = c = c \latminus a'$.
By monotonicity we have $ \Dfunapp{S_1}{a'} \join \Dfunapp{S_2}{c \latminus a' } \cgeq
\Dfunapp{S_1}{a} \join  \Dfunapp{S_2}{c \latminus a }$ as wanted. Suppose  $c \latminus a' \cl c$
holds. In this case, which is more interesting,  we can build a poset 
$L = (\{ a' \join c, \ a', \ c, \ c \latminus a', \ a' \meet (c \latminus a')\ \}, \cleq)$
and verify that $L$ is a non-distributive sub-lattice of $({\Con},\cleq)$, isomorphic
to a lattice known as $\mathbf{N}_5$ (see Fig.~\ref{ex:n5}). But from order theory
we know this cannot happen since we assumed $({\Con},\cleq)$ to be distributive,
and distributive lattices do not have sub-lattices isomorphic to $\mathbf{N}_5$
(\cite{davey2002introduction}).
\end{proof}

\begin{figure}[t]
 \centering
 \resizebox{0.3\textwidth}{!}{%
 \begin{tikzpicture}
  \node [shape = circle, draw] (A) at (0,0.5)  {$a$};
  \node [shape = circle, draw] (B) at (-2,2) {$b$};
  \node [shape = circle, draw] (C) at (-2,4) {$c$};
  \node [shape = circle, draw] (D) at (0,5.5)  {$d$};
  \node [shape = circle, draw] (E) at (2,3)  {$e$};

  \draw (A) to node {} (B);
  \draw (A) to node {} (E);
  \draw (B) to node {} (C);
  \draw (C) to node {} (D);
  \draw (D) to node {} (E);
 \end{tikzpicture}
 }%
 \caption{Non-distributive lattice: $\mathbf{N}_5$.}
 \label{ex:n5}
\end{figure}


==> tex-if-root.tex <==
% !TEX root = ./main.tex


